Dynamic Hub-and-Spoke Memory for Streaming Video Understanding

Streaming video understanding requires answering questions at arbitrary times over a continuously growing visual stream. The central challenge is to compactly remember long-range history while effectively retrieving question-relevant evidence. We propose Dynamic Hub-and-Spoke Memory (D-HSM), a training-free framework that represents distant history as structured textual memory while preserving the recent frames as visual tokens for fine-grained perception. Specifically, D-HSM turns selected historical video chunks into typed textual observations and stores them in an entity-centered hub-and-spoke memory, with entities as hubs and related evidence as spokes. When answering a question, D-HSM dynamically retrieves a compact question-aware memory subset, expands it through hub-and-spoke links, and combines it with the recent visual window for frozen-VLM answer prediction. Extensive experiments on both streaming and long video benchmarks show that D-HSM consistently and substantially improves VLM backbones and outperforms other state-of-the-art online and offline video understanding baselines.

==> figs/case1.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/assets/case1.pdf}
    \caption{\textbf{Visualization of hub-and-spoke memory details and the integrated retrieval context for the question from StreamingBench.}}
    \label{fig:case1}
\end{figure*}

==> figs/case2.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/assets/case2.pdf}
    \caption{\textbf{Visualization of hub-and-spoke memory details and the integrated retrieval context for the question from StreamingBench.}}
    \label{fig:case2}
\end{figure*}

==> figs/case3.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/assets/case3.pdf}
    \caption{\textbf{Visualization of hub-and-spoke memory details and the integrated retrieval context for the question from OVO-Bench.}}
    \label{fig:case3}
\end{figure*}

==> figs/case4.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/assets/case4.pdf}
    \caption{\textbf{Visualization of hub-and-spoke memory details and the integrated retrieval context for the question from OVO-Bench.}}
    \label{fig:case4}
\end{figure*}

==> figs/chunk.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{latex/assets/chunk.pdf}
    \caption{\textbf{Ablation on the historical observation budget on OVO-Bench} (Qwen2.5-VL-7B, 4 recent frames).}
    \label{fig:chunk}
\end{figure}

==> figs/hs.tex <==
\begin{figure*}[t]
    \vspace{-1mm}
    \centering
    \includegraphics[width=0.9\linewidth]{latex/assets/hs.pdf}
    \caption{\textbf{Example of the hub-and-spoke memory representation.}
Entities such as the ``artist'', ``canvas'', ``paintbrushes'', and ``sketch'' are stored as hubs with consistent identifiers, while their associated actions, spatial relations, OCR text, and events are stored as timestamped spokes.
Repeated or related evidence is attached to the corresponding entity hub, enabling D-HSM to localize and connect evidence across different moments in the video.}
    \label{fig:hs}
\end{figure*}

==> figs/motivation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{latex/assets/motivation.pdf}
    \caption{\textbf{Comparison of different historical strategies on OVO-Bench \cite{li2025ovobenchfarvideollmsrealworld}, measured by accuracy on ``Real-Time'' and ``Backward'' tasks.} The ``Static HSM Retrieval'' setting retrieves a fixed top-$K$ budget of memory entries for each question.``Real-Time'' means that the questions can be answered based on the recent video frames, while `Backward'' questions require evidence from history video chunks.}
    \label{fig:motivation}
\end{figure}

==> figs/similarity.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/assets/similarity.pdf}
    \caption{\textbf{Dynamic cutoff analysis for the question ``What does the person do after chopping the onion?''.}
The similarity scores quickly flatten after the high-similarity prefix.}
    \label{fig:similarity}
\end{figure}

==> figs/topk.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{latex/assets/topk.pdf}
    \caption{\textbf{Ablation on the maximum retrieval budget $K$ on OVO-Bench} (Qwen2.5-VL-7B, 4 recent frames).}
    \label{fig:topk}
\end{figure}

==> latex/algos/algo_all.tex <==
\begin{algorithm}[t]
\caption{Overall D-HSM Streaming Inference}
\label{alg:dhsm_overview}
\begin{algorithmic}[1]
\Require Historical chunks $\{h_t\}_{t=1}^{T}$; recent visual window $r_t$; question $q_t$
\Require History budget $B$; retrieval budget $K$; threshold $\theta$; gap parameters $\lambda_0,\lambda_1$
\Ensure Answer $a_t$ when question $q_t$ arrives
\State Initialize memory $M_0 \gets \emptyset$ and active set $\mathcal{S}_0 \gets \emptyset$
\For{$t=1,\ldots,T$}
    \State $\mathcal{H}_t \gets \{h_1,\ldots,h_t\}$
    \State $\mathcal{S}_t \gets \mathcal{H}_t$ if $t \le B$, otherwise $\Pi_B(\mathcal{H}_t)$
    \State $\Delta_t^+ \gets \mathcal{S}_t \setminus \mathcal{S}_{t-1}$
    \State $\Delta_t^- \gets \mathcal{S}_{t-1} \setminus \mathcal{S}_t$
    \State $M_t \gets \Call{UpdateMemory}{M_{t-1},\Delta_t^+,\Delta_t^-}$ \Comment{Alg.~\ref{alg:dhsm_update}}
    \If{question $q_t$ arrives}
        \State $C_t \gets \Call{Retrieve}{M_t,q_t,K,\theta,\lambda_0,\lambda_1}$ \Comment{Alg.~\ref{alg:dhsm_retrieval}}
        \State $a_t \gets f_{\mathrm{VLM}}(C_t,r_t,q_t)$
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

==> latex/algos/algo_retrival.tex <==
\begin{algorithm}[t]
\caption{Dynamic Hub-and-Spoke Retrieval}
\label{alg:dhsm_retrieval}
\begin{algorithmic}[1]
\Require Memory $M_t$; question $q_t$; retrieval budget $K$;
base threshold $\theta$; gap parameters $\lambda_0,\lambda_1$
\Ensure Linearized textual context $C_t$
\Statex $\mathcal{X}_t\!=\!\mathcal{H}(M_t)\cup\mathcal{P}(M_t)$:
memory entries; $\phi$: text encoder
\Statex $\chi_{\mathrm{cur}},\chi_{\mathrm{time}}$:
current-state and time-aware query indicators
\Statex $\operatorname{TopK}_K$: top-$K$ by score;
$\operatorname{sort}_{\downarrow}$: descending score sort
\Statex $\Gamma_{\mathrm{sp}},\Gamma_{\mathrm{co}},
\Gamma_{\mathrm{temp}}$: spoke, co-occurrence, and temporal-link expansion
\Statex $\mathcal{T}$: timestamp augmentation;
$\operatorname{Lin}$: textual linearization
\If{$\chi_{\mathrm{cur}}(q_t)=1$}
    \State \Return $C_t\gets\emptyset$
\EndIf
\State $s(e)\gets\cos\!\left(\phi(q_t),\phi(e)\right),
\ \forall e\in\mathcal{X}_t$
\State $\mathcal{A}_t\gets
\operatorname{TopK}_K\{e\in\mathcal{X}_t:s(e)\geq\theta\}$
\State $\{(e_i,s_i)\}_{i=1}^{n}\gets
\operatorname{sort}_{\downarrow}
\{(e,s(e)):e\in\mathcal{A}_t\}$
\If{$n<2$}
    \State $k_t\gets n$
\Else
    \State $\Delta_i\gets s_i-s_{i+1},
    \quad i\in\{1,\ldots,n-1\}$
    \State $i^\star\gets\arg\max_i\Delta_i,
    \quad \Delta^\star\gets\Delta_{i^\star}$
    \State $\gamma_t\gets
    \max\!\left(\lambda_0,\lambda_1[s_1-\theta]_+\right)$
    \If{$\Delta^\star\geq\gamma_t\ \land    \Delta^\star\geq2\,\operatorname{median}_i(\Delta_i)$}
        \State $k_t\gets i^\star$
    \Else
        \State $k_t\gets n$
    \EndIf
\EndIf
\State $\mathcal{E}_t\gets\{e_i\}_{i=1}^{k_t}$
\State $\widehat{\mathcal{E}}_t\gets
\mathcal{E}_t\cup\Gamma_{\mathrm{sp}}(\mathcal{E}_t)$
\State $\widehat{\mathcal{E}}_t\gets
\widehat{\mathcal{E}}_t\cup
\Gamma_{\mathrm{co}}(\widehat{\mathcal{E}}_t)\cup
\Gamma_{\mathrm{temp}}(\widehat{\mathcal{E}}_t)$
\If{$\chi_{\mathrm{time}}(q_t)=1$}
    \State $\widehat{\mathcal{E}}_t\gets
    \widehat{\mathcal{E}}_t\cup
    \mathcal{T}(\widehat{\mathcal{E}}_t)$
\EndIf
\State $C_t\gets\operatorname{RenderText}(\widehat{\mathcal{E}}_t)$
\State \Return $C_t$
\end{algorithmic}
\end{algorithm}

==> latex/algos/algo_update.tex <==
\begin{algorithm}[t]
\caption{Hub-and-Spoke Memory Update}
\label{alg:dhsm_update}
\begin{algorithmic}[1]
\Require Previous memory $M_{t-1}$; added chunks $\Delta_t^+$;
removed chunks $\Delta_t^-$; entity-linking threshold $\tau_{\mathrm{link}}$
\Ensure Updated memory $M_t$
\Statex $\mathcal{X}(M)=\mathcal{H}(M)\cup\mathcal{P}(M)\cup
\mathcal{E}^{\mathrm{co}}(M)\cup\mathcal{E}^{\mathrm{temp}}(M)$
\Statex $\mathcal{I}(c)=\{x\in\mathcal{X}(M):c\in\mathrm{supp}(x)\}$
\State $M_t \gets M_{t-1}$
\ForAll{$c\in\Delta_t^-,\;x\in\mathcal{I}(c)$}
    \State $\mathrm{supp}(x)\gets\mathrm{supp}(x)\setminus\{c\}$
\EndFor
\State $M_t\gets M_t\setminus
\{x\in\mathcal{X}(M_t):\mathrm{supp}(x)=\emptyset\}$
\State $(n_x,T_x)\gets
\bigl(|\mathrm{supp}(x)|,\{t(c):c\in\mathrm{supp}(x)\}\bigr),
\ \forall x\in\mathcal{X}(M_t)$
\State $a(p)\gets\arg\max_{v\in\mathcal{H}(M_t)}
\cos\!\left(\phi(p),\phi(v)\right),
\ \forall p:a(p)\notin\mathcal{H}(M_t)$
\State $(\mathcal{E}^{\mathrm{co}},\mathcal{E}^{\mathrm{temp}})
\gets\Psi_{\mathrm{rel}}(M_t)$
\ForAll{$h_j\in\Delta_t^+$}
    \State $z_j\gets\phi_{\mathrm{obs}}(h_j)$
    \State $\mathcal{N}_j\gets
    z_j[\textsc{People}\cup\textsc{Objects}]$
    \State $\mathcal{P}_j\gets
    z_j[\textsc{Actions}\cup\textsc{OCR-Text}\cup
    \textsc{Spatial}\cup\textsc{Event}]$
    \ForAll{$u\in\mathcal{N}_j$}
        \State $(v^\star,s^\star)\gets
        \operatorname{NN}\!\left(\phi(u),\mathcal{H}(M_t)\right)$
        \If{$s^\star\geq\tau_{\mathrm{link}}$}
            \State $\operatorname{id}(u)\gets\operatorname{id}(v^\star)$
        \Else
            \State $v^\star\gets\operatorname{NewHub}(u)$
            \State $M_t\gets M_t\cup\{v^\star\}$
        \EndIf
        \State $\mathrm{supp}(v^\star)\gets
        \mathrm{supp}(v^\star)\cup\{h_j\}$
    \EndFor
    \ForAll{$p\in\mathcal{P}_j$}
        \If{$\operatorname{IDs}(p)\neq\emptyset$}
            \State $a(p)\gets
            \{v:\operatorname{id}(v)\in\operatorname{IDs}(p)\}$
        \Else
            \State $a(p)\gets\arg\max_{v\in\mathcal{H}(M_t)}
            \cos\!\left(\phi(p),\phi(v)\right)$
        \EndIf
        \State $p^\star\gets\operatorname{MergeOrInsert}(p,M_t)$
        \State $\mathrm{supp}(p^\star)\gets
        \mathrm{supp}(p^\star)\cup\{h_j\}$
    \EndFor
    \State $\mathcal{E}^{\mathrm{co}}\gets
    \mathcal{E}^{\mathrm{co}}\cup\Psi_{\mathrm{co}}(\mathcal{N}_j,h_j)$
    \State $\mathcal{E}^{\mathrm{temp}}\gets
    \mathcal{E}^{\mathrm{temp}}\cup\Psi_{\mathrm{temp}}(\mathcal{P}_j,h_j)$
    \State $\mathcal{I}(h_j)\gets
    \{x\in\mathcal{X}(M_t):h_j\in\mathrm{supp}(x)\}$
\EndFor
\State \Return $M_t$
\end{algorithmic}
\end{algorithm}

==> latex/figs/method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/assets/method.pdf}
    \caption{\textbf{Overview of D-HSM.}
Historical chunks are converted by a frozen VLM into structured textual observations and incrementally organized into a dynamic hub-and-spoke memory.
When a question arrives, D-HSM dynamically retrieves a compact question-adaptive subset from memory and expands it through hub-and-spoke links.
Then, it combines the retrieved textual evidence with the recent visual tokens for frozen-VLM answer prediction.}
    \label{fig:framework}
\end{figure*}

==> latex/sec/1_intro.tex <==
\section{Introduction}
\input{latex/figs/motivation}


\begin{quote}
\textit{``Remembering is not the re-excitation of innumerable fixed, lifeless and fragmentary traces. It is an imaginative reconstruction, or construction.''}\par
\hfill --- Frederic C. Bartlett
\end{quote}



Streaming video understanding faces a memory problem in Bartlett's sense: the model must reconstruct question-relevant evidence rather than merely replay
the past.  
The requirement arises because a vision-language model (VLM) needs
access to long-range visual evidence, while the continuously growing video
history makes it infeasible to preserve the entire stream in raw visual form.
%
This raises a central question: \textit{how can a streaming model compactly remember the past while efficiently retrieving the evidence?}


Existing streaming video methods largely approach history from a token-budget perspective, reducing the past through sparse token selection~\citep{yao2025timechat,shu2025video,wu2019adaframe}, visual-token compression~\citep{wu2024longvideobenchbenchmarklongcontextinterleaved,li2025videoscanenablingefficientstreaming}, bounded memory banks~\citep{zhang2024flashvstreammemorybasedrealtimeunderstanding,wang2026streammecolongtermagentmemory}, or retrieval over cached visual representations~\citep{di2025streamingvideoquestionansweringincontext,yang2025streammemqueryagnostickvcache}. 
%
While these mechanisms improve online efficiency, they mainly ask \emph{which} past visual units should be retained, but leave open \emph{how} the retained history should be represented and organized for future questions.
%
A simple diagnostic in \cref{fig:motivation} illustrates the representation gap: appending historical video tokens (B) is less effective than converting the same segments into textual captions (C).
%
This suggests that converting distant history into textual semantic traces can provide a useful way to retain it under a limited context budget.
%
Yet flat captions remain segment-level summaries and lack explicit links among recurring entities, actions, and relations across time.
%
Therefore, the following question naturally arises: \fancynumber{1} \textit{How should a streaming model organize long-range history into structured semantic memory?}

Besides, different streaming questions require different evidence.
%
As shown in \cref{fig:motivation}, questions about the current moment are often better answered from the recent visual window alone (A), while adding historical context (B, C, D) can introduce irrelevant entities or events and distract the VLM.
%
In contrast, backward-looking or temporal questions require evidence from earlier segments, and cannot be answered reliably without retrieving history.
%
A useful memory must therefore not only be well-organized, but also be queried adaptively.
%
It should retrieve little or no history for real-time questions, and recover sufficient evidence for questions that depend on the past.
%
Thus, along with question \fancynumber{1}, another question needs to be answered for streaming video understanding: \fancynumber{2} \textit{How should a streaming model dynamically retrieve question-relevant history?}


To address both questions, we propose \textbf{\textit{D-HSM}}, a training-free \textbf{D}ynamic \textbf{H}ub-and-\textbf{S}poke \textbf{M}emory framework for streaming video understanding.
%
D-HSM handles the asymmetry between long history and the current moment by storing distant history as compact textual memory, while keeping the recent window as visual frames for fine-grained perception.
%
% Therefore, semantic abstraction is used where raw frames are no longer affordable, and fine-grained perception is preserved where it matters. 
%
For long-range history, D-HSM first converts selected historical video chunks into structured textual observations that describe visible entities and their associated evidence.
It then organizes these observations into an \textit{entity-centered hub-and-spoke memory}, where recurring entities serve as \textbf{hubs} and related evidence is attached as \textbf{spokes}.
This design turns flat segment captions into structured memory traces, allowing evidence about the same entity to be accumulated, merged, and localized across time.

When answering a question, D-HSM does not replay history in temporal order. Instead, it dynamically retrieves and constructs the relevant evidence on demand.
%
It first applies keyword-based gating to determine whether memory retrieval is needed.
When retrieval is triggered, D-HSM selects a memory subset according to the similarity between the question and memory entries.
%
Notably, rather than using a fixed top-$K$ budget, D-HSM determines the retrieval size by detecting a salient cutoff.
%
It then expands the selected subset through the hub-and-spoke structure.
%
The retrieved textual evidence of the subset is then combined with the recent visual tokens and passed to a frozen VLM for answer prediction.
As illustrated by \cref{fig:motivation}, D-HSM reconstructs question-relevant evidence from structured history while avoiding distraction from unnecessary historical information.
%

Together, the structured hub-and-spoke memory and the question-adaptive retrieval give a frozen VLM a way to remember the past compactly and access it selectively, without any additional training.
%
Extensive experiments show that D-HSM achieves state-of-the-art performance on streaming benchmarks such as StreamingBench \cite{lin2024streamingbenchassessinggapmllms} and OVO-Bench \cite{li2025ovobenchfarvideollmsrealworld}, outperforming strong proprietary models, as well as open-source online and offline video understanding baselines.
%
Meanwhile, D-HSM also retains strong performance on conventional offline long-video understanding benchmarks, including LongVideoBench \cite{wu2024longvideobenchbenchmarklongcontextinterleaved}, MLVU \cite{zhou2025mlvubenchmarkingmultitasklong}, and VideoMME \cite{fu2025videommefirstevercomprehensiveevaluation}.
% Ablation studies further confirm the effectiveness of the proposed hub-and-spoke memory and dynamic retrieval design.
These results demonstrate the robustness and generality of D-HSM for compactly remembering long video history and retrieval question-relevant evidence on demand.

% Together, the structured hub-and-spoke memory and the question-adaptive retrieval give a frozen VLM a way to remember the past compactly and access it selectively, without any additional training. We evaluate D-HSM on \TODO{benchmark names} under streaming video understanding settings, where it \TODO{headline result 1, e.g., consistently improves over strong streaming baselines} and \TODO{headline result 2, e.g., particularly benefits questions that require long-range or temporal reasoning, while remaining competitive on real-time questions}. \TODO{optional one-line ablation takeaway, e.g., Ablations further confirm that both the structured memory and the dynamic retrieval are necessary, and that naive flat-caption memory or fixed-budget retrieval underperforms D-HSM by a clear margin.}
% Our contributions are summarized as follows:
% \begin{itemize}
%     \item We identify two key memory challenges in streaming video understanding: how to organize long-range history into structured semantic memory, and how to dynamically retrieve question-relevant history.
%     \item We propose D-HSM, a training-free framework that represents long-range history as an entity-centered hub-and-spoke textual memory while preserving the recent visual window for fine-grained perception.
%     \item We introduce dynamic hub-and-spoke retrieval, which adaptively selects memory evidence for each question and expands it through entity, co-occurrence, and temporal-action links.
%     \item Experiments on \TODO{benchmark names} show that D-HSM improves over \TODO{baseline types}, with ablations validating the contributions of structured memory and dynamic retrieval.
% \end{itemize}




==> latex/sec/2_related.tex <==
\section{Related Work}
\input{figs/method}

\textbf{Long and Streaming Video Understanding.}
Recent methods address long-range temporal reasoning mainly by retaining or compressing visual tokens. Offline long-video models~\citep{chen2025longvila,wang2024longllava,shu2025video,song2024moviechat,wang2024videoagent,corona2025vlogger,lin2026unleashing} extend visual context by sampling more frames or scaling representations, but their computational costs grow rapidly with video length. Some methods organize events into graph memories, retrieving only query relevant subgraph to reduce the cost~\citep{chu2025understanding,huang2026buildingmindpalacestructuring,malik2026ravu}. They are primarily evaluated in offline  settings rather than under streaming queries. 
%

%
Online or streaming approaches~\citep{chen2024videollm,huang2024online,zeng2026streamforest,carreira2017quo,feichtenhofer2019slowfast,bertasius2021space,arnab2021vivit,liu2026graph2video,zhangprogressive} instead process frames sequentially. To manage history, sampling-based compression~\citep{yao2025timechat,shu2025video,wu2019adaframe,liu2025keyframe} reduces input tokens but discards fine-grained spatial or temporal details. Alternatively, storage-based compression~\citep{zeng2026streamforest,gu2024mamba,sun2024hawk,wang2025accelerating,li2024videomamba,he2024ma, zheng2026pearl} maintains visual memory after encoding. 
These methods largely retain history as features without explicitly organizing the relationship between different entities.
% This makes it difficult to reconstruct question-relevant history on demand.
D-HSM instead maintains a persistent, entity-centric memory that is incrementally updated as chunks arrive, enabling compact and question adaptive retrieval.

% D-HSM instead stores distant history as an entity-centered hub-and-spoke memory, enabling compact and question-adaptive retrieval.


\noindent \textbf{Video Large Language Models.}
Video Large Language Models (Video-LLMs) map spatiotemporal visual features into LLM spaces to enable open-ended dialogue and reasoning~\cite{maaz2024video,lin2024video,wang2024internvideo2,li2023blip,liu2024llava,achiam2023gpt,xiao2026staying}. Standard architectures establish modality alignment via abstractors~\cite{li2023blip,ye2023mplug,zhao2024thinimg}, projection layers~\cite{liu2024llava,zhu2023minigpt,li2026rethinking,xiao2026adapting}, or temporal pooling operators~\cite{zhang2023video} over established vision backbones~\cite{radford2021learning,fang2023eva,zhao2026hieramp,zhao2026s2dit}. Recent variants optimize efficiency via dynamic resolution encoding~\cite{bai2025qwen} and parameter-efficient tuning~\cite{hu2021lora,xiao2026not,zhang2025sensitivity}.
%
% To alleviate dense visual redundancy, token acceleration paradigms that merge tokens via visual clustering~\cite{bolya2022tome,yang2024dynamic,han2025holitom,zhao2026s2dit}.
% and intra-LLM configurations that use text-to-visual attention for query-adaptive token pruning~\cite{chen2025fastv,acl2025prunevid}. 
% However, these foundational models explicitly rely on a rigid visual-token-centric design.

==> latex/sec/3_method.tex <==
\section{Method}
\input{latex/figs/hs}

\subsection{Framework}
For the streaming video understanding, we require balance two forms of evidence: long-range historical context and immediate perception \cite{zeng2026streamforest, lin2024streamingbenchassessinggapmllms, qian2024streaminglongvideounderstanding}.
%
These two information streams are inherently asymmetric, as long-range history is too voluminous to retain in raw form, while the present moment demands fine-grained visual detail that resists lossy abstraction.
%
Building on this observation, we propose Dynamic Hub-and-Spoke Memory (D-HSM), a training-free framework that preserves recent video evidence as visual frames and consolidates longer-range history into a textual hub-and-spoke memory of compact semantic traces.

%
Specifically, as shown in Figure~\ref{fig:framework}, D-HSM maintains a textual memory $M_t$ for the historical stream.  
At each streaming step $t$, the historical chunk $h_t$ is converted into a typed textual observation $z_t$, which is incrementally integrated into the entity-centered hub-and-spoke memory:
\[
z_t = \phi_{\mathrm{obs}}(h_t), \quad
M_t = \mathcal{U}(M_{t-1}, z_t), 
\]
where $M_t$ is the textual hub-and-spoke memory accumulated up to step $t$. 


% Specifically, as shown in Figure~\ref{fig:framework} \TODO{figure}, D-HSM maintains a textual memory $M_t$ for the historical video chunks $\mathcal{H}_t=\{h_1,\ldots,h_{N_t}\}$.
% Each selected historical chunk $h_j$ is converted into a typed textual observation:
% \[
% z_j = \phi_{\mathrm{obs}}(h_j),
% \]
% where $\phi_{\mathrm{obs}}$ is a frozen-VLM observation function.
% The observations are then integrated into the entity-centered hub-and-spoke memory:
% \[
% M_t = \mathcal{U}(M_{t-1}, \Delta_t^+, \Delta_t^-),
% \]
% where $\Delta_t^+$ and $\Delta_t^-$ denote the chunk additions and removals induced by the current historical observation budget, and $\mathcal{U}$ updates the active memory accordingly.
% Thus, $M_t$ stores the compact textual evidence accumulated for the currently selected historical chunks.









%
Questions may arrive at arbitrary streaming steps. When a question $q_t$ arrives at step $t$, D-HSM dynamically selects a compact question-aware hub-and-spoke evidence subset $C_t$ from the current memory $M_t$ and combines it with the recent visual window $r_t$:
\[
C_t = \mathcal{R}(M_t, q_t), \quad
a_t = f_{\mathrm{VLM}}(C_t, r_t, q_t),
\]
where $\mathcal{R}$ denotes dynamic hub-and-spoke retrieval, $f_{\mathrm{VLM}}$ is the frozen VLM used for answer prediction, and $a_t$ is the predicted answer.

\subsection{D-HSM Construction and Update}
\label{sec:method-memory}
D-HSM constructs the historical textual memory $M_t$ in three stages: (i) it dynamically selects a bounded set of historical video chunks, (ii) it converts the selected chunks into structured textual observations, and (iii) it integrates these observations into an entity-centered Hub-and-Spoke memory.


\noindent\textbf{Dynamic Historical Observation Budget.}
Before constructing memory, D-HSM adapts the density of historical observations to the length of the available video prefix. 
%
We construct historical chunks by uniformly sampling frames from the video, with each sampled frame treated as the representative of one chunk.
%
Let $\mathcal{H}_t=\{h_1,\ldots,h_t\}$ be the candidate historical chunks at step $t$.
D-HSM selects an active observation set:
\[
\mathcal{S}_t =
\begin{cases}
\mathcal{H}_t, & t \le B,\\
\Pi_B(\mathcal{H}_t), & t > B,
\end{cases}
\]
where $B$ is the history budget and $\Pi_B(\cdot)$ denotes approximately uniform selection of $B$ chunks from $\mathcal{H}_t$.
%
As the video grows, the change in the active set is:
\[
\Delta_t^+ = \mathcal{S}_t \setminus \mathcal{S}_{t-1}, \quad
\Delta_t^- = \mathcal{S}_{t-1} \setminus \mathcal{S}_t .
\]
D-HSM generates textual observations only for chunks in $\Delta_t^+$, and excludes evidence supported only by chunks in $\Delta_t^-$ from the active memory.
This allows short prefixes to be represented densely, while longer prefixes are represented by a sparser set of semantic traces.

\noindent\textbf{Structured Textual Observations.} 
For each selected historical chunk, D-HSM applies a fixed-schema prompt (details in \appcref{app:observation-template}) to instruct a frozen VLM, yielding a textual observation: \textsc{Objects}, \textsc{People}, \textsc{Actions}, \textsc{OCR-Text}, \textsc{Spatial}, and \textsc{Event}.
%
% \textsc{Objects} and \textsc{People} assign distinct identifiers to different visible entities ($O_1, O_2, \ldots$ for objects and $P_1, P_2, \ldots$ for people), and reuse the same identifier for the same entity across different chunks.
\textsc{Objects} and \textsc{People} produce chunk-level entity mentions with local identifiers and concise visual descriptions. Across different chunks, D-HSM merges mentions of the same entity into a single persistent identity based on the similarity of their visual descriptions.
%
\textsc{Actions} describes interactions among these entities, \textsc{OCR-Text} captures screen text across optical character recognition, \textsc{Spatial} records positional relations, and \textsc{Event} summarizes the main event in the current chunk.

The schema converts each chunk into typed evidence rather than an unstructured caption.  
Persistent entity identifiers make it easier to track the same person or object across chunks by assigning each visible entity a unique symbol, such as $P_i$ or $O_i$, and reusing the same symbol whenever that entity reappears.
%
The remaining fields preserve complementary evidence in separable forms.  
Together, these typed observations expose the information needed for later memory construction and retrieval.

\noindent\textbf{Entity Hub-Centered Memory Construction and Update.} 
As shown in \cref{fig:hs}, D-HSM is organized around \emph{entity hubs} instantiated from \textsc{Objects} and \textsc{People}, which provide anchors for \emph{who} or \emph{what} is tracked across time.
% Formally, we represent the memory as:
% \[
% M_t = (\mathcal{V}_t, \mathcal{P}_t, \mathcal{E}^{\mathrm{co}}_t, \mathcal{E}^{\mathrm{temp}}_t),
% \]
% where $\mathcal{V}_t$ is the set of entity hubs, $\mathcal{P}_t$ is the set of typed spokes, $\mathcal{E}^{\mathrm{co}}_t$ stores co-occurrence edges between entities, and $\mathcal{E}^{\mathrm{temp}}_t$ stores temporal edges between action spokes.
%
Other chunk-level evidence types are stored as \emph{spokes} attached to the relevant entity hubs. 
These spokes answer \emph{what happened}, \emph{where it happened}, and \emph{when it was observed}.  
%
Besides, each hub and spoke also stores its timestamps and occurrence count, allowing D-HSM to localize evidence in time.
% and update an existing memory entry whenever the same entity or fact reappears.
%



As illustrated in \cref{fig:framework}, D-HSM updates the Hub-and-Spoke memory online.
For each incoming observation at time $t$, it applies the following rules:
% (i) \textit{Entity update.} If the observation mentions an existing entity identifier, D-HSM updates the corresponding hub instead of creating a duplicate. The hub refreshes its timestamps, and increments its occurrence count.  If the identifier has not appeared before, a new entity hub is created.
\textit{(i) Entity linking and hub update.}
For each newly observed entity, D-HSM compares its description embedding with the embeddings of existing entity hubs using cosine similarity. If the similarity to the closest hub exceeds $\tau_{\mathrm{link}}$, the entity is merged into that hub and reuses its persistent identifier. Otherwise, a new hub is created. The
resulting hub then records the supporting chunk and timestamp.
%
\textit{(ii) Spoke insertion and merging.} For spokes that mention entity identifiers such as \textit{P1} or
\textit{O2}, D-HSM attaches the spoke to the corresponding entity hub.
%
When the spoke text does not mention any entity identifier, D-HSM compares the spoke embedding with existing entity-hub embeddings, and links it to the most similar hub.
Then, D-HSM updates existing spokes for repeated facts by refreshing their timestamps and occurrence count, while inserting novel facts as new spokes.
% %
\textit{(iii) Local relational update.} Entities that appear in the same chunk are connected with co-occurrence edges.  These edges record local entity context, so retrieving one entity can also surface other entities observed in the same chunk.
\textit{(iv) Temporal action update.} For each entity hub, D-HSM links action spokes according to their observation order. These edges record the local order of actions performed by the same entity, so a retrieved action can bring in neighboring actions performed by the same entity.
\textit{(v) Support-based memory removal.}
D-HSM records the supporting chunks for each memory element and
maintains an inverted index from chunks to their contributions.
When a chunk in $\Delta_t^{-}$ is removed, D-HSM deletes its support,
recomputes the affected counts and timestamps, and removes elements
with no remaining support. Spoke attachments and relational edges
are then updated using the remaining observations, preventing stale
evidence from remaining in memory.





\subsection{Dynamic Hub-and-Spoke Retrieval}
\label{sec:method-retrieval}

Given the current memory $M_t$ and query $q_t$, D-HSM retrieves a compact, question-aware subset of the Hub-and-Spoke memory rather than passing the entire memory to the VLM.  
Retrieval proceeds in two steps: query-adaptive evidence selection and hub-and-spoke evidence expansion.

\noindent\textbf{Question-Adaptive Evidence Selection.}
D-HSM first uses a lightweight keyword-based gate to skip memory retrieval for explicitly current-state questions (e.g., cues such as \textit{now}, \textit{currently}, or \textit{recent frame}).
%
For history-dependent questions, D-HSM embeds the query $q_t$ and the memory entries, and computes cosine similarity scores. 
%
After applying a base threshold $\theta$ and a maximum budget $K$, we obtain a ranked candidate list
$\{(e_i,s_i)\}_{i=1}^{n}$, where $s_i \ge s_{i+1}$ and $n \le K$.
%
D-HSM truncates this list at the most prominent \emph{score gap}, when such a gap is statistically distinguishable from the rest of the distribution. Specifically, we examine the gaps:
\[
\Delta_i = s_i - s_{i+1}, \quad i = 1, \ldots, n-1,
\]
and locate the largest one, $\Delta^\star = \Delta_{i^\star}$ with $i^\star = \arg\max_i \Delta_i$.
%
We accept $i^\star$ as the truncation point only if $\Delta^\star$ passes two tests. First, it must exceed a confidence-adaptive threshold:
\[
\gamma_t = \max\!\big(\lambda_0,\; \lambda_1[s_1 - \theta]_+\big), \quad [x]_+ = \max(x, 0),
\]
where $\lambda_0$ is an absolute floor and the second term tightens the threshold when the top score $s_1$ is high, so that a sharper gap is required when the retriever is confident. Second, $\Delta^\star$ must be at least twice the median gap, $\Delta^\star \ge 2\,\mathrm{median}(\{\Delta_i\})$, which rules out cases where scores decay smoothly and no single gap is genuinely salient.
%
When both tests pass, we set $k_t = i^\star$; otherwise (including the degenerate case $n < 2$) we fall back to $k_t = n$. D-HSM then retrieves $\mathcal{E}_t = \{e_i\}_{i=1}^{k_t}$.


% Given a threshold $\theta$, a maximum budget $K$, and a gap threshold $\gamma$, D-HSM selects: 
% \[
% k_t =
% \min\left(
% K,\;
% \min \{ i : s_i \ge \theta \ \text{and}\ s_i - s_{i+1} \ge \gamma \}
% \right),
% \]
% and retrieves $\mathcal{E}_t=\{e_i\}_{i=1}^{k_t}$.  
% If no clear gap is found, $k_t$ defaults to the number of entries above $\theta$, capped by $K$.  
% This dynamic retrieval gives simple questions concise evidence while preserving more context for ambiguous or multi-entity questions.

\input{latex/table/sb}

\noindent\textbf{Hub-and-Spoke Evidence Expansion.}
Given the selected evidence entries $\mathcal{E}_t$, D-HSM expands them using the Hub-and-Spoke structure of the memory.  
For an entity hub, the expansion includes its attached spokes, together with entities that co-occurred in the same chunk as discussed in \cref{sec:method-memory}. 
Notably, when attaching action spokes, D-HSM follows a short next-action chain to recover neighboring actions performed by the same entity. For time-aware questions, it also retrieves timestamped events from the stored timeline.

Then, the resulting evidence set is linearized into a textual context with entity-centered profiles, screen-text snippets, chronological event lines, and counting aggregates as illustrated in \cref{tab:rendered-context}. 
This context is then combined with the recent visual frames and the query for frozen-VLM.



==> latex/sec/4_experiment.tex <==
\section{Experiments}
\input{latex/table/ovo}
\subsection{Implementation Details.}
D-HSM is training-free and keeps all VLM parameters frozen.
We use Qwen2.5-VL-7B \cite{bai2025qwen25vltechnicalreport} and Qwen3-VL-8B as backbone models \cite{bai2025qwen3vltechnicalreport}.
%
For each video, we use $20$ historical chunks by default to construct the hub-and-spoke memory.
% Each selected chunk is converted into a structured textual observation with the fixed prompt in \appcref{app:observation-template}.
%
We set 4 recent frames and  dynamic retrieval with a maximum budget of $K=12$ as default setting.
Memory entries and questions are embedded with a lightweight embedding encoder (bge-small-en-v1.5) \cite{bge_embedding}, and the dynamic cutoff gap $\lambda_0=0.05, \lambda_1=0.12$.
All experiments are conducted on NVIDIA RTX A6000 GPUs without any task-specific fine-tuning.

\subsection{Performance Comparison.}

\noindent\textbf{Streaming Video Understanding.} 
~\cref{tab:video_results} and~\cref{tab:results} report results on StreamingBench \cite{lin2024streamingbenchassessinggapmllms} and OVO-Bench \cite{li2025ovobenchfarvideollmsrealworld}.
%
Across both benchmarks, \textit{all D-HSM variants consistently outperform other methods}.
%
On StreamingBench, D-HSM raises the overall score from 73.7 to 84.7 using Qwen2.5-VL, and further reaches 85.4 with Qwen3-VL.
%
D-HSM surpasses the strongest proprietary model, Gemini 1.5 Pro, and the strongest open-source online model, Streamforest, by 9.7 and 8.1 points, respectively.
%
The improvement suggests that the gains are not tied to a particular backbone, but are closely related to how D-HSM represents and retrieves long-range history.

On OVO-Bench, the improvement is not limited to a single question type: D-HSM achieves competitive results across Real-Time Visual Perception, Backward Tracing, and Forward Active Responding tasks.
%
This indicates that D-HSM can dynamically adapt its evidence use, relying on the recent visual window for current-state questions while retrieving historical evidence for questions that require earlier moments.


\noindent\textbf{Offline Long Video Understanding.}
~\cref{tab:video_benchmarks_reorg} evaluates D-HSM on offline long-video understanding benchmarks, including LongVideoBench \cite{wu2024longvideobenchbenchmarklongcontextinterleaved}, MLVU \cite{zhou2025mlvubenchmarkingmultitasklong}, and VideoMME \cite{fu2025videommefirstevercomprehensiveevaluation}.
%
% Beyond the streaming setting, D-HSM also provides robust performance in offline long-video understanding.
%
With Qwen2.5-VL as the backbone, D-HSM achieves 60.7 on LongVideoBench, 67.3 on MLVU, and 63.9 on VideoMME, outperforming the Qwen2.5-VL baseline and several open-source long-video models.
%
% Compared with online baselines, D-HSM performs better than Dispider and TimeChatOnline on LongVideoBench and VideoMME, while remaining competitive on MLVU.
%
% These results suggest that the proposed hub-and-spoke memory is not limited to streaming queries.
%
This shows that, beyond the streaming setting, D-HSM can serve as an effective compact representation for long-range evidence in offline long-video understanding.


\input{latex/table/long}

\subsection{Ablation Study}

\noindent\textbf{Effect of Memory Sources.}
\input{latex/table/hub_or_recent_ovo}
~\cref{tab:ablation_hub_recent_ovo} compares the two evidence sources in D-HSM.
Recent frames preserve real-time visual details, whereas HSM provides stronger historical evidence.
Combining them yields the best backward score without sacrificing real-time accuracy, showing that recent perception and long-range memory are necessary.

\noindent\textbf{Effect of Memory Organization.}
\input{latex/table/memory_organization}
~\cref{tab:ablation_memory_organization} ablates how historical observations are organized.
Typed observations improve the quality over flat chronological captions, and entity-centered organization provides better results. 
Besides, the D-HSM organization provides further gains, with each component making a meaningful contribution. 
%
Removing co-occurrence edges, next-action chains, or spoke merging consistently reduces performance, confirming that these components provide complementary temporal and relational evidence.

\noindent\textbf{Effect of Dynamic Retrieval.}
\input{latex/table/dynamic}
We compare the proposed dynamic retrieval strategy with a fixed top-$K$ strategy that always retrieves the maximum number 12 of memory entries.
%
As shown in ~\cref{tab:ablation_topk_dynamic}, dynamic retrieval improves performance on both benchmarks, indicating that adapting retrieval to different question types is beneficial.
%
% Moreover, because dynamic retrieval does not always use the full top-$K$ budget, it reduces the average number of retrieved tokens by \TODO{X\%}, thereby lowering inference cost.
% \TODO{efficiency compare}
%

\noindent\textbf{Effect of Retrieval Budget.}
We vary the maximum retrieval budget $K$ to study how much memory evidence should be made available during retrieval.
As shown in \cref{fig:topk}, performance improves as $K$ increases from 4 to 12, suggesting that a larger budget helps recover supporting long-range evidence.
%
However, further increasing $K$ to 16 does not bring additional gains and slightly reduces performance.
This suggests that retrieving more memory entries is not always beneficial, since weakly related evidence may introduce unnecessary tokens and distract the model.
The result further supports the need for adapting the amount of retrieved evidence instead of always using a larger fixed budget.

\noindent\textbf{Effect of Historical Observation Budget.}
We vary the historical observation budget by changing the number of chunks used to construct memory.
As shown in \cref{fig:chunk}, performance first improves as the budget increases, reaching the top with 20 chunks.
%
This indicates that a larger historical budget can provide broader temporal coverage and preserve more useful long-range evidence.
%
However, further increasing the budget to 25 or 30 chunks reduces performance.
We attribute this drop to redundant or weakly relevant historical observations, which can introduce noise into memory and make retrieval less focused.
These results suggest that D-HSM benefits from a moderate historical budget that balances coverage and compactness.


\input{latex/figs/topk}

\input{latex/figs/chunk}


==> latex/sec/5_analysis.tex <==
\section{Analysis}
\label{sec:analysis}

\subsection{Inference Efficiency Analysis}
\input{latex/table/latency_memory}
We measure the end-to-end cost of D-HSM on 50 StreamingBench samples using a single Nvidia A100 GPU.
\cref{tab:efficiency} separates background streaming ingestion from the latency after a question arrives.
Observation generation dominates ingestion at 1.55 seconds per selected chunk, whereas the structural memory update takes 49 ms and removed-chunk handling takes only 0.6 ms per rotation.
%
Video ingestion and memory processing are streamed, so subsequent chunks can arrive while the current selected chunk is being processed. Because the processing is much faster than it accumulates, preventing any long-term backlog.
%
At question time, retrieval takes 11 ms and answer generation takes 0.74 seconds, giving a question-path latency of approximately 0.75 seconds.
Thus, the hub-and-spoke memory operations add little overhead; most computation comes from the frozen VLM used for observation and answer generation.

\subsection{Dynamic Cutoff Analysis}
\input{latex/figs/similarity}
We analyze the top-12 question--memory similarities to explain the behavior of dynamic retrieval.
As shown in \cref{fig:similarity}, a short high-similarity prefix is followed by a much flatter score distribution.
D-HSM cuts off retrieval at this gap instead of always retaining all 12 candidates, thereby filtering weakly related entries before hub-and-spoke expansion.
This keeps the evidence compact, reduces distraction from marginal historical context, and lowers the average number of retrieved tokens by about 51\% on OVO-Bench.

\subsection{Memory Quality Analysis}
\input{latex/table/memory_quality}
To evaluate the intermediate memory independently, we conduct a comprehensive quantitative evaluation of D-HSM’s key components using human annotations. We randomly sampled 30 videos from StreamingBench and manually annotated by human: (i) 100 pairs of temporally distinct entity mentions that D-HSM merged into the same hub, (ii) 170 entity hubs, and (iii) 96 spoke-to-hub attachments. The 100 mentioned pairs span 90 distinct hubs. 
As shown in \cref{tab:memory_quality}, the accuracy are computed by comparing D-HSM outputs produced with Qwen2.5-VL against human judgments as ground truth. The results identify that the structured memory is reasonably reliable.

\subsection{Failure Cases Analysis}
We manually assign 100 incorrect predictions to mutually exclusive primary causes.
The complete breakdown is reported in \cref{tab:failure_analysis}. The largest source is answer synthesis by the frozen VLM (31\%), followed by observation generation (23\%) and retrieval (19\%).
It shows that in D-HSM, the main bottleneck is evidence selection rather than graph expansion. 
%
Entity linking accounts for another 10\% of failures, consistent with the memory quality evaluation above.
We find that most of them are predictive questions, because such questions often contain weak entity-specific cues.


==> latex/sec/5_conclusion.tex <==
\section{Conclusion}
We presented D-HSM, a training-free framework that balances long-range memory and immediate perception for streaming video understanding.
%
D-HSM stores distant history as entity-centered hub-and-spoke textual memory while keeping recent frames for fine-grained perception.
%
Its dynamic retrieval selects and expands question-relevant evidence on demand, reducing unnecessary historical context.
%
Experiments on streaming and offline long-video benchmarks show that D-HSM outperforms existing online and offline baselines.
%
These results highlight the value of reconstructing the past through structured, question-aware memory.

==> latex/table/ablation_history_graph.tex <==
\begin{table}[t!]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Ablation study on OVO-Bench. We highlight our method with \colorbox{cyan!10}{cyan background}.}
\label{tab:ablation}

\begin{tabular}{lcc}
\toprule
\textbf{Setting} & \textbf{Real-Time} & \textbf{Backward} \\
\midrule

Recent Frames (4f)
& \cellcolor{cyan!10}\textbf{78.98} 
& 58.34 \\

+ History Video Frames (20f)
& 75.06 
& 52.89 \\

+ History Text Caption (20f)
& 76.81 
& 53.91 \\

+ Hub and Spoke Memory (20f)
& 77.11 
& \cellcolor{cyan!10}\textbf{62.82} \\

\bottomrule
\end{tabular}
\end{table}

==> latex/table/chunk.tex <==
\begin{table}[t]
\centering
\small
\caption{
Effect of different chunk sizes on OVO Bench using Qwen2.5-VL-7B.
}
\resizebox{\columnwidth}{!}{

\begin{tabular}{lc}
\toprule
\textbf{Chunk Size} & \textbf{OVO Bench} \\
\midrule
10 & 66.20 \\
15 & 66.59 \\
20 & 66.84 \\
25 & 66.20 \\
30 & 66.13 \\
\bottomrule
\end{tabular}
}

\label{tab:chunk_size_ovo}
\end{table}

==> latex/table/k.tex <==
\begin{table}[t]
\centering
\small
\caption{Effect of the maximum retrieval budget $K$ on OVO-Bench using Qwen2.5-VL-7B with 4 recent frames.}
\resizebox{\columnwidth}{!}{

\begin{tabular}{lc}
\toprule
\textbf{Dynamic Top-$k$} & \textbf{OVOBench} \\
\midrule
4  &  66.37\\
8  &  66.41\\
12 &  66.84\\
16 &  66.82\\
\bottomrule
\end{tabular}
}

\label{tab:qwen_topk_ovobench}
\end{table}

==> latex/table/long_old.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\caption{Evaluation results on video benchmarks with explicit model size.}
\setlength{\tabcolsep}{6pt} % 7列布局，稍微放大列间距让排版更舒展
\begin{tabular}{l c | c c c c c}
\toprule
\textbf{Model} & \textbf{Size} & \textbf{MVBench} & \textbf{PerceptionTest} & \textbf{LongVideoBench} & \textbf{MLVU} & \textbf{VideoMME} \\
 & & (Avg.) & (Val) & (Val) & (M-Avg) & (w/o subs) \\
\cmidrule(lr){1-7}
\multicolumn{2}{l}{Video Duration (Avg.)} & 16s & 23s & 473s & 651s & 1010s \\
\midrule

\multicolumn{7}{c}{\textsc{Proprietary Models}} \\

GPT-4o          & -- & 64.6 & --   & 66.7 & 64.6 & 71.9 \\
Gemini 1.5 Pro  & -- & 60.5 & --   & 64.0 & --   & 75.0 \\
\midrule

\multicolumn{7}{c}{\textsc{Open-Source Models}} \\
LongVA & 7B & -- & -- & -- &56.3 &52.6 \\
Kangaroo       & 8B & 61.0 & --   & 54.8 & 61.0 & 56.0 \\
% LongVILA       & 7B & --   & --   & --   & --   & 57.5 \\
LongVU         & 7B & 66.9 & --   & --   & 65.4 & 60.6 \\
Apollo         & 7B & --   & 67.3 & 58.5 & 70.9 & 61.3 \\

SF-LLaVA-1.5   & 7B & --   & 69.6 & 62.5 & 71.5 & 63.9 \\
InternVL2.5    & 8B & 72.0 & 68.2 & 60.0 & 68.9 & 64.2 \\
NVILA          & 8B & 68.1 & 65.4 & 57.7 & 70.1 & 64.2 \\
% VideoChat-Flash & 7B & 74.0 & 76.2 & 64.7 & 74.7 & 65.3 \\
VideoLLaMA3    & 7B & 69.7 & 72.8 & 59.8 & 73.0 & 66.2 \\
\midrule
% Dispider & 7B & 

\textbf{Qwen2.5-VL+Ours } & 7B & &  & 60.7  & 70.3 &  63.9  \\ 

\bottomrule
\end{tabular}

\label{tab:video_benchmarks_reorg}
\end{table*}

==> sec/0_abstract.tex <==
\begin{abstract}
Streaming video understanding requires answering questions at arbitrary times over a continuously growing visual stream.
%
The central challenge is to compactly remember long-range history while effectively retrieving question-relevant evidence.
%
We propose \textbf{D}ynamic \textbf{H}ub-and-\textbf{S}poke \textbf{M}emory \textbf{(D-HSM)}, a \textit{training-free} framework that represents distant history as structured textual memory while preserving the recent frames as visual tokens for fine-grained perception.
%
Specifically, D-HSM turns selected historical video chunks into typed textual observations and stores them in an entity-centered hub-and-spoke memory, with entities as hubs and related evidence as spokes.
%
When answering a question, D-HSM dynamically retrieves a compact question-aware memory subset, expands it through hub-and-spoke links, and combines it with the recent visual window for frozen-VLM answer prediction.
%
Extensive experiments on both streaming and long video benchmarks show that D-HSM consistently and substantially improves VLM backbones and outperforms other state-of-the-art online and offline video understanding baselines.
% Ablation studies further validate the importance of structured memory, recent visual perception, and dynamic retrieval for reconstructing question-relevant evidence in streaming videos.
\end{abstract}

% \TODO{1. the red todo 2. check algorithm  3. appendix algorithm  4. efficiency/memory  5. estimate tokens}

==> table/ablation_history_graph.tex <==
\begin{table}[t!]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Ablation study on OVO-Bench. We highlight our method with \colorbox{cyan!10}{cyan background}.}
\label{tab:ablation}

\begin{tabular}{lcc}
\toprule
\textbf{Setting} & \textbf{Real-Time} & \textbf{Backward} \\
\midrule

Recent Frames (4f)
& \cellcolor{cyan!10}\textbf{78.98} 
& 58.34 \\

+ History Video Frames (20f)
& 75.06 
& 52.89 \\

+ History Text Caption (20f)
& 76.81 
& 53.91 \\

+ Hub and Spoke Memory (20f)
& 77.11 
& \cellcolor{cyan!10}\textbf{62.82} \\

\bottomrule
\end{tabular}
\end{table}

==> table/chunk.tex <==
\begin{table}[t]
\centering
\small
\caption{
Effect of different chunk sizes on OVO Bench using Qwen2.5-VL-7B.
}
\resizebox{\columnwidth}{!}{

\begin{tabular}{lc}
\toprule
\textbf{Chunk Size} & \textbf{OVO Bench} \\
\midrule
10 & 66.20 \\
15 & 66.59 \\
20 & 66.84 \\
25 & 66.20 \\
30 & 66.13 \\
\bottomrule
\end{tabular}
}

\label{tab:chunk_size_ovo}
\end{table}

==> table/dynamic.tex <==
\begin{table}[t]
\centering
\small
\caption{
\textbf{Ablation on dynamic retrieval.}
We compare fixed top-$12$ retrieval with the proposed dynamic retrieval strategy, whose maximum retrieval budget is also set to 12 (Qwen2.5-VL-7B, 4 recent frames).
}
\resizebox{1.0\columnwidth}{!}{

\begin{tabular}{lcc}
\toprule
\textbf{Dataset} &
\textbf{Fixed Top-$k$} &
\textbf{Dynamic} \\
\midrule
OVO-Bench             &  64.71   & \textbf{66.84} \\
StreamingBench  & 79.47 & \textbf{82.45} \\
\bottomrule
\end{tabular}
}

\label{tab:ablation_topk_dynamic}

\end{table}

==> table/failure_analysis.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Primary causes of 100 manually analyzed failures.}
Indented rows decompose their parent categories and are not additional errors.
}
\resizebox{0.82\columnwidth}{!}{
\begin{tabular}{lc}
\toprule
\textbf{Error source} & \textbf{Percentage} \\
\midrule
Observation generation       & 23\% \\
\quad Recognition           & 21\% \\
\quad OCR                   & 2\% \\
Entity linking               & 10\% \\
Retrieval                    & 19\% \\
\quad Selection             & 19\% \\
\quad Expansion             & 0\% \\
Answer synthesis             & 31\% \\
Benchmark issues             & 17\% \\
\quad Ground-truth error    & 5\% \\
\quad Multiple valid answers & 12\% \\
\bottomrule
\end{tabular}
}
\label{tab:failure_analysis}
\end{table}

==> table/hub_or_recent_ovo.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Ablation of memory sources on OVO-Bench.}
We compare HSM only, recent frames only, and the full D-HSM.
All results use Qwen2.5-VL-7B; the recent visual window contains four frames when enabled.
}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
 & \textbf{Real-Time} & \textbf{Backward} \\
\midrule
HSM only                     & 44.79 & 58.02 \\
Recent frames only           & 78.98 & 55.66 \\
\rowcolor{cyan!7} Full D-HSM & \textbf{78.98} & \textbf{62.82} \\
\bottomrule
\end{tabular}
}
\label{tab:ablation_hub_recent_ovo}
\end{table}

==> table/k.tex <==
\begin{table}[t]
\centering
\small
\caption{Effect of the maximum retrieval budget $K$ on OVO-Bench using Qwen2.5-VL-7B with 4 recent frames.}
\resizebox{\columnwidth}{!}{

\begin{tabular}{lc}
\toprule
\textbf{Dynamic Top-$k$} & \textbf{OVOBench} \\
\midrule
4  &  66.37\\
8  &  66.41\\
12 &  66.84\\
16 &  66.82\\
\bottomrule
\end{tabular}
}

\label{tab:qwen_topk_ovobench}
\end{table}

==> table/latency_memory.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{\textbf{End-to-end efficiency of D-HSM.}
Average wall-clock time over 50 StreamingBench samples on a single A100.
Streaming costs are measured per selected chunk or memory rotation, whereas question-time costs are measured per question.
}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lc}
\toprule
\textbf{Stage} & \textbf{Average time} \\
\midrule
Observation generation & 1.55 s \\
Memory update          & 49 ms \\
Removed-chunk handling          & 0.6 ms \\
\midrule
Retrieval            & 11 ms \\
Answer generation          & 0.74 s \\
\bottomrule
\end{tabular}
}
\label{tab:efficiency}
\end{table}

==> table/long.tex <==
\begin{table}[t!]
\centering
\normalsize
\caption{\textbf{Evaluation results on offline long-video understanding benchmarks.}
We evaluate D-HSM on LongVideoBench \cite{wu2024longvideobenchbenchmarklongcontextinterleaved}, MLVU \cite{zhou2025mlvubenchmarkingmultitasklong}, and VideoMME \cite{fu2025videommefirstevercomprehensiveevaluation} against different methods. D-HSM results are reported with Qwen2.5-VL using 4 recent frames. 
}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l c | c c c}
\toprule
\textbf{Model} & \textbf{Size} & \textbf{LongVideoBench} & \textbf{MLVU} & \textbf{VideoMME} \\
 & & (Val) & (M-Avg) & (w/o subs) \\
\cmidrule(lr){1-5}
\multicolumn{2}{l}{Video Duration (Avg.)} & 473s & 651s & 1010s \\
\multicolumn{2}{l}{Video Length} & 8s -- 60min & 3min -- 120min & 1min -- 60min \\
\midrule

\multicolumn{5}{c}{\textsc{Proprietary Models}} \\

GPT-4o          & --    & 66.7 & 64.6 & 71.9 \\
Gemini 1.5 Pro  & --    & 64.0 & --   & 75.0 \\
\midrule

\multicolumn{5}{c}{\textsc{Open-Source Offline Models}} \\
LongVA & 7B  & -- &56.3 &52.6 \\
Kangaroo       & 8B  & 54.8 & 61.0 & 56.0 \\
% LongVILA       & 7B & --   & --   & --   & --   & 57.5 \\
LongVU         & 7B   & --   & 65.4 & 60.6 \\
Apollo         & 7B   & 58.5 & 70.9 & 61.3 \\

SF-LLaVA-1.5   & 7B   & 62.5 & 71.5 & 63.9 \\
InternVL2.5    & 8B   & 60.0 & 68.9 & 64.2 \\
NVILA          & 8B   & 57.7 & 70.1 & 64.2 \\
% VideoChat-Flash & 7B  & 64.7 & 74.7 & 65.3 \\
VideoLLaMA3    & 7B   & 59.8 & 73.0 & 66.2 \\
\midrule
\multicolumn{5}{c}{\textsc{Open-Source Online Models}} \\
Dispider       & 7B   & -- & 61.7 & 57.2 \\
Streamforest   & 7B   & -- & \textbf{69.6} & 61.9 \\
TimeChatOnline & 7B   &  \underline{57.7}  & 65.4 & \underline{62.5}\\

\rowcolor{cyan!7}\textbf{D-HSM} & 7B & \textbf{60.7}  & \underline{67.3} &  \textbf{63.9}  \\ 

\bottomrule
\end{tabular}
}

\label{tab:video_benchmarks_reorg}
\end{table}

==> table/long_old.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\caption{Evaluation results on video benchmarks with explicit model size.}
\setlength{\tabcolsep}{6pt} % 7列布局，稍微放大列间距让排版更舒展
\begin{tabular}{l c | c c c c c}
\toprule
\textbf{Model} & \textbf{Size} & \textbf{MVBench} & \textbf{PerceptionTest} & \textbf{LongVideoBench} & \textbf{MLVU} & \textbf{VideoMME} \\
 & & (Avg.) & (Val) & (Val) & (M-Avg) & (w/o subs) \\
\cmidrule(lr){1-7}
\multicolumn{2}{l}{Video Duration (Avg.)} & 16s & 23s & 473s & 651s & 1010s \\
\midrule

\multicolumn{7}{c}{\textsc{Proprietary Models}} \\

GPT-4o          & -- & 64.6 & --   & 66.7 & 64.6 & 71.9 \\
Gemini 1.5 Pro  & -- & 60.5 & --   & 64.0 & --   & 75.0 \\
\midrule

\multicolumn{7}{c}{\textsc{Open-Source Models}} \\
LongVA & 7B & -- & -- & -- &56.3 &52.6 \\
Kangaroo       & 8B & 61.0 & --   & 54.8 & 61.0 & 56.0 \\
% LongVILA       & 7B & --   & --   & --   & --   & 57.5 \\
LongVU         & 7B & 66.9 & --   & --   & 65.4 & 60.6 \\
Apollo         & 7B & --   & 67.3 & 58.5 & 70.9 & 61.3 \\

SF-LLaVA-1.5   & 7B & --   & 69.6 & 62.5 & 71.5 & 63.9 \\
InternVL2.5    & 8B & 72.0 & 68.2 & 60.0 & 68.9 & 64.2 \\
NVILA          & 8B & 68.1 & 65.4 & 57.7 & 70.1 & 64.2 \\
% VideoChat-Flash & 7B & 74.0 & 76.2 & 64.7 & 74.7 & 65.3 \\
VideoLLaMA3    & 7B & 69.7 & 72.8 & 59.8 & 73.0 & 66.2 \\
\midrule
% Dispider & 7B & 

\textbf{Qwen2.5-VL+Ours } & 7B & &  & 60.7  & 70.3 &  63.9  \\ 

\bottomrule
\end{tabular}

\label{tab:video_benchmarks_reorg}
\end{table*}

==> table/memory_context.tex <==
\begin{table*}[t]
\centering
\small
\caption{\textbf{Examples of textual evidence blocks rendered from D-HSM memory and provided to the VLM.}
The exact entries depend on the retrieved hubs, spokes, screen-text nodes, and timeline events.}
\begin{tabular}{p{0.22\linewidth} p{0.70\linewidth}}
\toprule
\textbf{Rendered block} & \textbf{Template shown to the VLM} \\
\midrule
Entity-centered profile &
\texttt{[P1 (blue-shirt woman)]}\\
& \texttt{\ \ [00:05] picks up O2 (red mug)}\\
& \texttt{\ \ [00:08] walks toward O3 (wooden table)}\\
\midrule
% Unlinked evidence &
% \texttt{[Other]}\\
% & \texttt{\ \ * [00:14] A person opens the door.} \\
% \midrule
Screen text &
\texttt{[Screen Text]}\\
& \texttt{\ \ * "EXIT"}\\
& \texttt{\ \ * "12:30"} \\
\midrule
Most recent events &
\texttt{[Most recent events]}\\
& \texttt{\ \ [00:21] The person leaves the room.}\\
& \texttt{\ \ [00:24] The door closes.} \\
\midrule
Timeline &
\texttt{[Timeline]}\\
& \texttt{\ \ [00:05] A woman picks up a red mug near the table.}\\
\midrule
Counting aggregate &
\texttt{[Counting Aggregate --- observed action occurrences across captioned chunks]}\\
& \texttt{\ \ 'place' (e.g. "P1 places O2 on O3"): 3 time(s) at [00:05, 00:08, 00:13]} \\
\bottomrule
\end{tabular}

\label{tab:rendered-context}
\end{table*}

==> table/memory_organization.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\caption{\textbf{Ablation of memory organization on OVO-Bench.}
We progressively replace flat captions with typed and entity-centered memory, and remove individual D-HSM components.
All results use Qwen2.5-VL-7B with four recent frames.
}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcc@{}}
\toprule
 & \textbf{Overall} & \textbf{Backward} \\
\midrule
Flat captions (chronological)                & 58.97 & 53.91 \\
Typed observations w/o entity organization  & 62.99 & 60.73 \\
Entity-centered memory only                  & 63.51 & 60.94 \\
\rowcolor{cyan!7} Full D-HSM               & \textbf{66.80} & \textbf{62.82} \\
\quad w/o co-occurrence edges              & 65.33 & 60.46 \\
\quad w/o next-action chains               & 65.48 & 60.69 \\
\quad w/o spoke merging                    & 66.28 & 61.56 \\
\bottomrule
\end{tabular}
}
\label{tab:ablation_memory_organization}
\end{table}

==> table/memory_quality.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Quality of the constructed memory.}
Human evaluation on 30 StreamingBench videos using Qwen2.5-VL-7B.
}
\resizebox{0.92\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Metric} & \textbf{Score} & \textbf{Samples} \\
\midrule
Entity-linking pair accuracy $\uparrow$ & 77.0\% & 100 pairs \\
Hub purity  $\uparrow$                 & 84.4\% & 90 hubs \\
Duplicate-hub rate $\downarrow$ & 8.8\% & 170 hubs \\
Spoke-attachment precision $\uparrow$  & 87.1\% & 96 spokes \\
\bottomrule
\end{tabular}
}
\label{tab:memory_quality}
\end{table}

==> table/nf.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation on the recent visual window size.}}
\footnotesize 
\resizebox{\columnwidth}{!}{
\begin{tabular}{l cccc} 
\toprule
 & \multicolumn{2}{c}{\textbf{OVO-Bench}} & \multicolumn{2}{c}{\textbf{StreamingBench}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} 
{\textbf{Recent}}& Qwen2.5 & Qwen3 & Qwen2.5 & Qwen3 \\
{\textbf{Frames}}& \scriptsize{(VL-7B)} & \scriptsize{(VL-8B)} & \scriptsize{(VL-7B)} & \scriptsize{(VL-8B)} \\
\midrule
2f & 64.93          & 64.01          & 80.46          & 81.18          \\
4f & \textbf{66.84} & \textbf{65.59} & 82.45          & 83.08          \\
6f & 66.53          & 64.69          & 83.42          & 84.86          \\
8f & 65.55          & 65.09          & \textbf{84.73} & \textbf{85.36} \\
\bottomrule
\end{tabular}
}
\label{tab:ablation_transpose_top_ours}
\end{table}
% \begin{table}[t]
% \centering
% \normalsize
% \resizebox{\columnwidth}{!}{ % 稍微加宽列间距，避免数据挤在一起
% \begin{tabular}{l cccc cccc} % 移除了所有纵向实体黑线
% \toprule
% \multirow{3}{*}{\textbf{Dataset}} & \multicolumn{8}{c}{\textbf{Ours}} \\
% \cmidrule(lr){2-9} % 第一层横线：覆盖后面全部8列
% & \multicolumn{4}{c}{\textbf{Qwen2.5-VL (7B)}} & \multicolumn{4}{c}{\textbf{Qwen3-VL (8B)}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} % 第二层横线：左右独立裁剪，中间自然断开留白
% & \textbf{2f} & \textbf{4f} & \textbf{6f} & \textbf{8f} & \textbf{2f} & \textbf{4f} & \textbf{6f} & \textbf{8f} \\
% \midrule
% OVO   & 64.93 & \textbf{66.84} & 66.53 & 65.55 & 64.01 & \textbf{65.59} & 64.69 & 65.09 \\
% StreamingBench & 80.46 & 82.45 & 83.42 & \textbf{84.73} & 81.18 & 83.08 & 84.86 & \textbf{85.36} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Ablation study on the number of frames across different base models.}
% \label{tab:ablation_transpose_top_ours}
% \end{table}

==> table/ovo.tex <==
\begin{table*}[t!]
\centering
\normalsize
\caption{\textbf{Comparison results of different methods on OVO-Bench \cite{li2025ovobenchfarvideollmsrealworld}.} }
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc|ccccccc|cccc|cccc|c}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{Size}\end{tabular}} & \multirow{2}{*}{\textbf{\#Frames}} & \multicolumn{7}{c|}{\textbf{Real-Time}} & \multicolumn{4}{c|}{\textbf{Backward}} & \multicolumn{4}{c|}{\textbf{Forward}} & \textbf{Overall} \\ 

\cmidrule(lr){4-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18}
 &  &  & OCR & ACR & ATR & STU & FPD & OJR & \textbf{Avg.} & EPM & ASI & HLD & \textbf{Avg.} & REC & SSR & CRR & \textbf{Avg.} & \textbf{Avg.} \\ 

\midrule
\rowcolor{gray!10}Human Agents & -  & - & 94.0 & 92.6 & 94.8 & 92.7 & 91.1 & 94.0 & 93.2 & 92.6 & 93.0 & 91.4 & 92.3 & 95.5 & 89.7 & 93.6 & 92.9 & 92.8\\
\midrule

\multicolumn{19}{c}{\textsc{Proprietary Models}} \\ 
GPT-4o & - & 64 & 69.8 & 64.2 & 71.6 & 51.1 & 70.3 & 59.8 & 64.5 & 57.9 & \underline{75.7} & 48.7 & 60.8 & 27.6 & \underline{73.2} & 59.4 & 53.4 & 59.5 \\ 
Gemini 1.5 pro & - & 1 fps & 85.9 & 67.0 & 79.3 & 58.4 & 63.4 & 62.0 & 69.3 & \underline{58.6} & \textbf{76.4} & 52.6 & \underline{62.5} & 35.5 & \textbf{74.2} & 61.7 & 57.2 & 63.0 \\
\midrule
\multicolumn{19}{c}{\textsc{Open-source Offline Models}} \\ 
LongVU & 7B & 1 fps & 53.7 & 53.2 & 62.9 & 47.8 & 68.3 & 59.8 & 57.6 & 40.7 & 59.5 & 4.8 & 35.0 & 12.2 & 69.5 & 60.8 & 47.5 & 46.7 \\
LLaVA-OV & 7B & 64 & 66.4 & 57.8 & 73.3 & 53.4 & 71.3 & 62.0 & 64.0 & 54.2 & 55.4 & 21.5 & 43.7 & 25.6 & 67.1 & 58.8 & 50.5 & 52.7 \\
LLaVA-Video & 7B & 64 & 69.1 & 58.7 & 68.8 & 49.4 & \underline{74.3} & 59.8 & 63.5 & 56.2 & 57.4 & 7.5 & 40.4 & 34.1 & 70.0 & 60.4 & 54.8 & 52.9 \\
Qwen2-VL & 72B & 64 & 65.8 & 60.6 & 69.8 & 51.7 & 69.3 & 54.4 & 61.9 & 52.5 & 60.8 & 57.5 & 57.0 & \textbf{38.8} & 64.1 & 45.0 & 49.3 & 56.3 \\
\midrule
\multicolumn{19}{c}{\textsc{Open-source Online Models}} \\ 
VideoLLM-online & 8B & 2 fps & 8.1 & 23.9 & 12.1 & 14.0 & 45.5 & 21.2 & 20.8 & 22.2 & 18.8 & 12.2 & 17.7 & - & - & - & - & - \\
Dispider & 8B & 1 fps & 57.7 & 49.5 & 62.1 & 44.9 & 61.4 & 51.6 & 54.6 & 48.5 & 55.4 & 4.3 & 36.1 & 18.1 & 37.4 & 48.8 & 34.7 & 41.8 \\
TimeChatOnline & 7B & 1 fps & 75.2 & 46.8 & 70.7 & 47.8 & 69.3 & 61.4 & 61.9 & 55.9 & 59.5 & 9.7 & 41.7 & 31.6 & 38.5 & 40.0 & 36.7 & 46.7 \\
Streamforest & 7B & 1 fps & 68.5 & 53.2 & 71.6 & 47.8 & 65.4 & 60.9 & 61.2 & \textbf{58.9} & 64.9 & 32.3 & 52.0 & 32.8 & 70.6 & 57.1 & 52.5 & 55.6 \\
Streamo & 7B & 1 fps & 77.2 & 66.1 & 76.7 & 45.5 & 66.3 & 72.8 & 67.4 & 55.6 & 58.1 & 33.9 & 49.2 & 30.8 & 57.6 & \textbf{82.5} & 57.0 & 57.9 \\

\midrule
% \textit{Qwen2.5-VL} & 7B & 20 &\multicolumn{16}{l}{} \\ 
\rowcolor{cyan!3}
\textit{Qwen2.5-VL}+ D-HSM (4f) & 7B & 20+4
& 94.0 & 70.7 & \textbf{86.2} & 66.9 & \textbf{75.3} & 81.0 & 79.0 
& 52.9 & 63.5 & \textbf{72.0} & \textbf{62.8} 
& \underline{36.4} & 71.9 & 67.1 & \underline{58.5} & \textbf{66.8} \\ 
\rowcolor{cyan!7}
\textit{Qwen2.5-VL}+ D-HSM (8f) & 7B & 20+8
& \textbf{96.0} & 73.4 & 81.0 & 66.3 & \textbf{75.3} & \underline{82.1} & 79.0 
& 52.2 & 60.8 & 62.4 & 58.5  
& \underline{36.4} & \textbf{74.2} & 67.1 & \textbf{59.2} & \underline{65.6} \\ 
% \textit{Qwen3-VL} & 8B & 20 & \multicolumn{16}{l}{} \\ 
\rowcolor{cyan!3}
\textit{Qwen3-VL}+ D-HSM (4f) & 8B & 20+4
& \underline{95.0} & \textbf{82.6} & \underline{84.5} & \textbf{72.5} & 71.3 & \textbf{83.7} & \textbf{81.6} 
& 54.6 & 62.2 & \underline{67.2} & 61.3
& 25.0 & 61.9 & \underline{74.6} & 53.8 & \underline{65.6} \\ 
\rowcolor{cyan!7}
\textit{Qwen3-VL}+ D-HSM (8f) & 8B & 20+8
& 94.0 & \underline{81.7} & 80.2 & \underline{67.4} & 72.3 & 81.5 & \underline{79.5} 
& 55.2 & 65.5 & 62.4 & 61.1  
& 24.9 & 64.7 & \underline{74.6} & 54.7 & 65.1\\
\bottomrule
\end{tabular}
}

\label{tab:results}
\end{table*}

==> table/sb.tex <==
\begin{table*}[t]
\centering
\normalsize
\caption{\textbf{Comparison results of different methods on StreamingBench  Real-Time
understanding tasks \cite{lin2024streamingbenchassessinggapmllms}.} D-HSM is evaluated with Qwen2.5-VL \cite{bai2025qwen25vltechnicalreport} and Qwen3-VL \cite{bai2025qwen3vltechnicalreport} using $4$ or $8$ recent frames, and compared with different proprietary, open-source offline, and open-source online video understanding models. ``20+4'' and ``20+8'' denote using 20 historical frames for memory construction and 4 or 8 recent frames for visual perception.}
\resizebox{\linewidth}{!}{
\begin{tabular}{llc|cccccccccc|c}
\toprule
\textbf{Model} & \textbf{Size} & \textbf{\#Frames} & \textbf{OP} & \textbf{CR} & \textbf{CS} & \textbf{ATP} & \textbf{EU} & \textbf{TR} & \textbf{PR} & \textbf{SU} & \textbf{ACP} & \textbf{CT} & \textbf{Overall} \\
\midrule
\rowcolor{gray!10}Human  & -  & - & 89.5 & 92.0 & 93.6 & 91.5 & 95.7 & 92.5 & 88.0 & 88.8 & 89.7 & 91.3 & 91.5\\
\midrule
\multicolumn{14}{c}{\textsc{Proprietary Models}} \\

GPT-4o         & -  & 64 & 77.1 & 80.5 & 83.9 & 76.5 & 70.2 & 83.8 & 66.7 & 62.2 & 69.1 & 49.2 & 73.3 \\
Claude 3.5 Sonnet  & -  & 20 & 80.5 & 77.3 & 82.0 & 81.7 & 72.3 & 75.4 & 61.1 & 61.8 & 69.3 & 43.1 & 72.4\\
Gemini 1.5 pro  & -  & 1 fps & 79.0 & 80.5 & 83.5 & 79.7 & \textbf{80.0} & 84.7 & 77.8 & 64.2 & 72.0 & 48.7 & 75.7 \\

\midrule
\multicolumn{14}{c}{\textsc{Open-source Offline Models}} \\

VILA-1.5     & 8B & 14 & 53.7 & 49.2 & 71.0 & 56.9 & 53.4 & 53.9 & 54.6 & 48.8 & 50.1 & 17.6 & 52.3 \\
LongVA       & 7B & 128 & 70.0 & 63.3 & 61.2 & 70.9 & 62.7 & 59.5 & 61.1 & 53.7 & 54.7 & 34.7 & 60.0 \\
MiniCPM-v2.6 & 7B & 32 & 71.9 & 71.1 & 77.9 & 75.8 & 64.6 & 65.7 & 70.4 & 56.1 & 62.3 & 53.4 & 67.4 \\
LLaVA-OneVision & 7B & 32 & 80.4 & 74.2 & 76.0 & 80.7 & 72.7 & 71.7 & 67.6 & 65.5 & 65.7 & 45.1 & 71.1 \\
\rowcolor{gray!10} Qwen2.5-VL    & 7B & 1 fps & 78.3 & 80.5 & 78.9 & 80.5 & 76.7 & 78.5 & 79.6 & 63.4 & 66.2 & 53.2 & 73.7 \\

\midrule
\multicolumn{14}{c}{\textsc{Open-source Online Models}} \\

Flash-VStream   & 7B & 1 fps & 25.9 & 43.6 & 24.9 & 23.9 & 27.3 & 13.1 & 18.5 & 25.2 & 23.9 & 48.7 & 23.2 \\
VideoLLM-online  & 8B & 2 fps & 39.1 & 40.1 & 34.5 & 31.1 & 46.0 & 32.4 & 31.5 & 34.2 & 42.5 & 27.9 & 36.0 \\
Dispider        & 8B & 1 fps & 74.9 & 75.5 & 74.1 & 73.1 & 74.4 & 59.9 & 76.1 & 62.9 & 62.2 & 45.8 & 67.6 \\
TimeChatOnline  & 7B & 1 fps & 80.2 & \underline{82.0} & 79.5 & 83.3 & 76.1 & 78.5 & 78.7 & 64.6 & 69.6 & \textbf{58.0} & 75.4 \\
Streamforest    & 7B & 1 fps & 83.1 & \textbf{82.8} & 82.7 & 84.3 & 77.5 & 78.2 & 76.9 & 69.1 & 75.6 & 54.4 & 77.3 \\

\midrule
% \textit{Qwen2.5-VL} & 7B & 20 & \multicolumn{11}{l}{} \\
\rowcolor{cyan!3}\textit{Qwen2.5-VL}+D-HSM (4f) & 7B  & 20+4 & {85.3} & {64.0} & {88.8} & {87.9} & {79.1} & {90.0} & {\textbf{87.6}} & \underline{79.7} & {79.6} & {47.8} & {82.5} \\
\rowcolor{cyan!7}\textit{Qwen2.5-VL}+D-HSM (8f) & 7B & 20+8 & 88.0 & 70.4 & \underline{93.1} & 88.2 & 78.5 & \textbf{93.8} & 81.9 & \textbf{80.9} & \underline{83.1} & 50.0 & \underline{84.7} \\
% \textit{Qwen3-VL} & 8B & 20 &\multicolumn{11}{l}{} \\
\rowcolor{cyan!3}\textit{Qwen3-VL}+D-HSM (4f) & 8B & 20+4 & \underline{86.9} & {64.8} & 92.1 & \underline{89.2} & {74.7} & {90.7} & \underline{85.7} & {77.6} & {79.6} & {54.5} & {83.1} \\
\rowcolor{cyan!7}\textit{Qwen3-VL}+D-HSM (8f) & 8B & 20+8 & \textbf{88.6} & {67.2} & \textbf{95.1} & \textbf{90.8} & \underline{79.8} & \underline{92.5} & \textbf{87.6} & 77.2 & \textbf{84.0} & \underline{55.6} & \textbf{85.4} \\
\bottomrule
\end{tabular}
}

\label{tab:video_results}
\end{table*}
